Towards General Purpose Vision Systems

Computer vision systems today are primarily N-purpose systems, designed and trained for a predefined set of tasks. Adapting such systems to new tasks is challenging and often requires non-trivial modifications to the network architecture (e.g. adding new output heads) or training process (e.g. adding new losses). To reduce the time and expertise required to develop new applications, we would like to create general purpose vision systems that can learn and perform a range of tasks without any modification to the architecture or learning process. In this paper, we propose GPV-1, a task-agnostic vision-language architecture that can learn and perform tasks that involve receiving an image and producing text and/or bounding boxes, including classification, localization, visual question answering, captioning, and more. We also propose evaluations of generality of architecture, skill-concept transfer, and learning efficiency that may inform future work on general purpose vision. Our experiments indicate GPV-1 is effective at multiple tasks, reuses some concept knowledge across tasks, can perform the Referring Expressions task zero-shot, and further improves upon the zero-shot performance using a few training samples.

==> figs/cfg.tex <==
\lstdefinelanguage{yaml}{
  keywords={true,false,null,y,n},
  keywordstyle=\color{darkgray}\bfseries,
  ndkeywords={},
  ndkeywordstyle=\color{black}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  %moredelim=[l]{}{:},
  comment=[l]{#},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{blue}\ttfamily,
  %morestring=[l]{-}{},
  morestring=[b]',
  morestring=[b]"
}

\begin{lstlisting}[language=yaml]
model:
  max_text_len: 20 # maximum number of words to sample during greedy decoding
  hidden_dim: 768
  roi_head: True
  relevance_conditioning: True
	
	# DETR params
  detr:
    num_queries: 100 # number of object queries
    num_classes: 1 # since box relevance is a binary classification problem
		
		# params for DETR's encoder-decoder
    hidden_dim: 256 
    nheads: 8
    num_encoder_layers: 6
    num_decoder_layers: 6
		
		# params for CNN backbone
    backbone: resnet50
    lr_backbone: ${training.lr_backbone}
		
		# other DETR params following official DETR implementation
    position_embedding: sine
    masks: False
    dilation: False
    dropout: 0.1
    dim_feedforward: 2048
    pre_norm: False
    aux_loss: False
    frozenbatchnorm: True
    last_layer_only: True # use only last layer features from DETR decoder
  
	# linear layer params before feeding DETR and BERT features into co-attention
	detr_joiner: 
    detr_dim: 256
    out_dim: ${model.hidden_dim}
  bert_joiner:
    bert_dim: 768
    out_dim: ${model.hidden_dim}
	
	# text decoder params
  text_decoder:
    hidden_dim: ${model.hidden_dim}
    dropout: ${model.detr.dropout}
    nheads: ${model.detr.nheads}
    pos_enc: False
    num_layers: 3
	
	# ViLBERT co-attention params
  co_att:
    visualization: False
    bi_num_attention_heads: 16
    bi_hidden_size: ${model.hidden_dim}
    hidden_size: ${model.hidden_dim}
    intermediate_size: 3072
    output_size: ${model.hidden_dim}
    attention_probs_dropout_prob: ${model.detr.dropout}
    hidden_dropout_prob: ${model.detr.dropout}
    hidden_act: gelu
    v_hidden_size: ${model.hidden_dim}
    v_intermediate_size: 3072
    v_output_size: ${model.hidden_dim}
    v_attention_probs_dropout_prob: ${model.detr.dropout}
    v_hidden_dropout_prob: ${model.detr.dropout}
    v_hidden_act: gelu
    num_layers: 3

  losses: ${losses}

# Essentially just two kinds of losses to minimize: 
# - Negative log-likelihood (NLL) of GT text (implemented using cross-entropy)
# - Hungarian Loss (for tasks with bounding box supervision)
#
# Captioning, VQA, Classification use cross-entropy
# Localization uses Hungarian loss (following official DETR implementation)
losses:
  CaptionLoss:
    name: caption_criterion
    loss_wts:
			# lower weight as captions have more words than answers or class names
      loss_caption: 5e-2 
  
  VqaLoss:
    name: vqa_criterion
    loss_wts:
      loss_vqa: 1
  
  ClsLoss:
    name: cls_criterion
    loss_wts:
      loss_cls: 1

  Localization:
    name: localization_criterion
		
		# cost weights used for hungarian matching of GT and predicted boxes
    cost_wts:
      ce: 1
      bbox: 5
      giou: 2
		
		# weights used for different losses after hungarian assignment
    loss_wts:
      loss_ce: 1
      loss_bbox: 5
      loss_giou: 2

		# lower weight used for background category in loss_ce to tackle imbalance
    eos_coef: 0.1

    num_classes: ${model.detr.num_classes}

training:
  frozen_epochs: 10 # DETR modules frozen for first 10 epochs
  num_epochs: 40 # total number of epochs
  batch_size: 120 # batch size
  lr: 1e-4 # maximum learning rate for all params except CNN backbone
  lr_backbone: 1e-5 # maximum learning rate used for CNN backbone
  weight_decay: 1e-4

	# lr goes from 0 to max in lr_warmup_fraction*num_epochs epochs
  lr_warmup: True 
  lr_warmup_fraction: 0.1
	
	# after warmup, lr goes from max to 0 in remaining epochs
	lr_linear_decay: True

  clip_max_norm: 0.1 # gradient clipping for DETR modules
\end{lstlisting}

==> figs/tab_our_split_single_task_comparison.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\begin{tabular}{lcccc}
                                  & \cellcolor[HTML]{E6B8AF}VQA       & \cellcolor[HTML]{FFF2CC}Cap.        & \cellcolor[HTML]{CFE2F3}Loc. & \cellcolor[HTML]{D9D2E9}Class. \\
\multicolumn{1}{r}{1-Task Baseline} & \multicolumn{1}{c}{\textbf{56.6}} & 0.832                               & 62.4                         & 75.2                           \\
\multicolumn{1}{r}{1-Task GPV}      & \multicolumn{1}{c}{55.9}          & \textbf{0.855} & \textbf{64.8}                & \textbf{75.3}                  \\
                                    &                                   & \multicolumn{1}{l}{}                & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          
\end{tabular}
\vspace{-0.2in}
\caption{
\label{tab:our_single_task_comparison}
\textbf{Comparison to special purpose baselines (\cocogpv\ split)}: When trained and tested on individual tasks, our architecture performs similarly to competent specialized architectures. 
}
\end{table}

==> figs/teaser.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=\textwidth]{figs/teaserv3.pdf}
\caption{
\label{fig:teaser} {\bf Teaser.} 
}
\end{figure*}

==> figs/vqa_heatmap.tex <==
\begin{figure*}[h!]
\centering
\includegraphics[width=0.99\textwidth,trim=0 10 0 10,clip]{figs/vqa_heatmap_pdf.pdf}
\vspace{-0.15in}
\caption{
\label{fig:vqa_heatmap} {\bf Skill-Concept generalization in VQA:} The percentage improvement of \model\ over 1-task \model\ on the various categories and question types of VQA (\cocogpv-test), if there are over 20 questions of that type and category. Multi-task training clearly helps most question types and categories, particularly question types that require skills from localization and classification (``how many'', ``where'', ``what is'') and categories $\in$ \hvqacap\ (concepts unseen during VQA training).
}
\vspace{-0.1in}
\end{figure*}
